EchoSpec: Training Search Agents to Weigh Evidence Above Echoes

Search agents trained with reinforcement learning decide what to retrieve, when to search again, and when to answer. In real corpora, one claim is copied and paraphrased across many pages while the primary source settling a question appears once. We show that reinforcement-learned search agents grant echoes the credence of independent sources and lose their ability to abstain. Across five base models from 3B to 32B and seven released RL agents on multi-hop Wikipedia questions with primary evidence intact, eight paraphrased false-claim echoes overturn 58-73% of previously correct answers, while exact-match RL drives deleted-evidence abstention below 15%. Conditioning on retrieval localizes the failure to evidence acquisition: once primary evidence enters context, agents overrule eight echoes as reliably as one, whereas echoes fill top ranks and halt search early, so larger budgets, forced search turns, or passive passage filtering alone fail to recover displaced evidence. We introduce EchoSpec, specifying reliability across five corpus transformations with known target answers and training in two stages. Verification warm-start teaches multi-hop bridge-entity recovery past echoes, after which group RL optimizes an evidence-gated $\lambda$-reward with an outcome-independent acquisition bonus and scale-preserving advantages retaining the optimal rule $\lambda/(1+\lambda)$. Across Qwen2.5-3B, Qwen2.5-7B, and Llama-3.1-8B backbones on nine evaluation suites, EchoSpec cuts eight-echo deference by 30-44 points on Qwen2.5-7B down to 29-31%, nearly quadruples eight-echo reach to 26-27% with zero-shot transfer to unseen BGE and BM25 retrievers, and raises standalone QA precision to 47-55%. Code is publicly available at https://github.com/unihsy/EchoSpec.

==> sections/table_ablation.tex <==
    \rowcolor{oursbg}\textbf{\method{} (default, $\eta{=}0$, 3 seeds)} & 14.3 & 28.9 & 25.8 & 31.3 & 16.7 & 37.6 & 47.1 & 40.1 \\
    \midrule
    \hspace{0.55em}w/o Stage~2 RL (warm-start only, 3 seeds) & 20.8 & 47.2 & 21.0 & 23.4 & 13.9 & 33.1 & 47.0 & 41.5 \\
    \hspace{0.55em}w/o Stage~1 warm-start ($\lambda$-RL only, 1 seed) & 45.4 & 69.4 & 9.4 & 9.2 & 5.2 & 32.5 & 42.4 & 37.6 \\
    \hspace{0.55em}w/o wrong-answer penalty ($\lambda{=}0$, 1 seed) & 12.9 & 29.3 & 28.7 & 32.2 & 19.5 & 20.6 & 42.3 & 39.6 \\
    \hspace{0.55em}w/o evidence gate ($\alpha{=}1$, 1 seed) & 16.8 & 31.1 & 26.5 & 26.3 & 16.9 & 39.6 & 50.0 & 41.6 \\
    \hspace{0.55em}w/o acq.\ bonus ($\beta_{\text{acq}}{=}0$, 1 seed) & 16.2 & 29.1 & 26.2 & 30.1 & 15.8 & 40.7 & 49.7 & 41.7 \\
    \hspace{0.55em}w/o exclude-seen retrieval (3 seeds) & 17.0 & 31.6 & 22.5 & 25.8 & 15.2 & 40.3 & 47.9 & 40.1 \\
    \hspace{0.55em}+ cross-world baseline ($\eta{=}0.35$, 3 seeds) & 12.8 & 31.5 & 27.4 & 29.9 & 16.1 & 31.6 & 43.3 & 37.6 \\
    \hspace{0.55em}w/o 32B teacher (self-guided 7B, 2 seeds) & 19.8 & 51.5 & 23.5 & 27.7 & 11.4 & 36.9 & 42.9 & 36.8 \\
    \hspace{0.55em}w/o 32B teacher \& acq.\ bonus (3 seeds) & 21.7 & 56.0 & 20.5 & 24.7 & 9.0 & 43.1 & 44.1 & 37.2 \\


==> sections/table_app_backbones.tex <==
    \rowcolor{grpbg}\multicolumn{9}{l}{\cellcolor{grpbg}\emph{Qwen2.5-3B-Instruct (3B parameters, cross-scale, 1 seed)}} \\
    \hspace{0.55em}No defense & 40.7 & 67.0 & 62.5 & 5.1 & 2.8 & 36.3 & 26.0 & 22.9 \\
    \hspace{0.55em}No defense (+ exclude-seen) & 44.5 & 61.5 & 65.2 & 4.7 & 2.4 & 37.0 & 26.4 & 23.3 \\
    \hspace{0.55em}TrustRAG & 38.9 & 39.9 & \runnerup{27.2} & 7.8 & 4.4 & 37.6 & 25.7 & 22.1 \\
    \hspace{0.55em}Exact-match RL & 42.7 & 69.4 & 71.5 & 11.6 & 5.3 & 5.2 & 35.1 & 34.6 \\
    \hspace{0.55em}Warm-start only & 18.3 & 35.5 & 39.1 & 19.3 & 11.7 & 25.2 & 40.7 & 36.7 \\
    \hspace{0.55em}\textbf{\method{}} & 15.3 & 29.6 & 30.4 & 22.5 & 12.4 & 37.5 & 42.8 & 36.9 \\
    \arrayrulecolor[HTML]{CBD2D9}\midrule\arrayrulecolor{black}
    \hspace{0.55em}\textbf{\method{}} + TrustRAG & 15.8 & 23.5 & \runnerup{12.3} & 23.5 & 15.6 & 38.6 & 42.1 & 36.4 \\
    \hspace{0.55em}\textbf{\method{}} + Sem.\ dedup & 20.6 & 34.6 & 34.5 & 30.1 & 14.5 & 36.6 & 42.7 & 36.9 \\
    \midrule
    \rowcolor{grpbg}\multicolumn{9}{l}{\cellcolor{grpbg}\emph{Qwen2.5-7B-Instruct (7B parameters, 3-seed \method{})}} \\
    \hspace{0.55em}No defense & 41.9 & 57.2 & 58.8 & 7.1 & 5.5 & \runnerup{49.2} & 41.1 & 33.8 \\
    \hspace{0.55em}No defense (+ exclude-seen) & 41.0 & 57.8 & 60.1 & 7.6 & 5.7 & 48.5 & 41.4 & 34.3 \\
    \hspace{0.55em}TrustRAG & 35.4 & 41.7 & \best{22.8} & 11.4 & 9.4 & 48.0 & 40.3 & 33.0 \\
    \hspace{0.55em}Exact-match RL (1 seed) & 35.2 & 59.5 & 67.7 & 15.9 & 8.1 & 1.4 & 37.2 & 36.8 \\
    \hspace{0.55em}Warm-start only (3 seeds) & 20.8 & 35.0 & 47.2 & 21.0 & 13.9 & 33.1 & 47.0 & 41.5 \\
    \hspace{0.55em}\textbf{\method{}} (3 seeds) & \runnerup{14.3} & \best{23.9} & 28.9 & \runnerup{25.8} & \runnerup{16.7} & 37.6 & \runnerup{47.1} & 40.1 \\
    \arrayrulecolor[HTML]{CBD2D9}\midrule\arrayrulecolor{black}
    \hspace{0.55em}\textbf{\method{}} + TrustRAG (3 seeds) & 13.8 & \runnerup{19.4} & 12.8 & 29.4 & 19.0 & 36.5 & 44.1 & 38.3 \\
    \hspace{0.55em}\textbf{\method{}} + Sem.\ dedup (3 seeds) & 16.7 & 25.9 & 28.7 & \runnerup{36.2} & 20.2 & 33.9 & 46.2 & 40.0 \\
    \midrule
    \rowcolor{grpbg}\multicolumn{9}{l}{\cellcolor{grpbg}\emph{Llama-3.1-8B-Instruct (8B parameters, cross-family, 1 seed)}} \\
    \hspace{0.55em}No defense & 37.3 & 67.5 & 70.0 & 10.8 & 3.8 & 5.0 & 28.4 & 27.6 \\
    \hspace{0.55em}No defense (+ exclude-seen) & 34.7 & 71.8 & 74.4 & 11.1 & 4.2 & 4.2 & 26.6 & 25.9 \\
    \hspace{0.55em}TrustRAG & 37.6 & 52.1 & 28.2 & 17.1 & 7.6 & 4.8 & 27.7 & 26.8 \\
    \hspace{0.55em}Exact-match RL & 33.8 & 61.3 & 66.7 & 17.6 & 9.8 & 2.8 & 42.7 & 42.2 \\
    \hspace{0.55em}Warm-start only & 22.7 & 35.2 & 45.7 & 21.0 & 14.6 & 24.7 & 45.5 & \runnerup{42.3} \\
    \hspace{0.55em}\textbf{\method{}} & \best{11.1} & \runnerup{24.1} & 30.6 & \best{26.5} & \best{17.2} & \best{52.5} & \best{55.4} & \best{44.2} \\
    \arrayrulecolor[HTML]{CBD2D9}\midrule\arrayrulecolor{black}
    \hspace{0.55em}\textbf{\method{}} + TrustRAG & 11.2 & \best{19.2} & \best{11.8} & 28.7 & \runnerup{20.8} & \runnerup{52.8} & 55.3 & 43.6 \\
    \hspace{0.55em}\textbf{\method{}} + Sem.\ dedup & 17.1 & 26.9 & 26.6 & \best{36.4} & \best{20.9} & \best{54.2} & \best{55.9} & \best{44.4} \\


==> sections/table_app_fairness.tex <==
    \rowcolor{grpbg}\multicolumn{9}{l}{\cellcolor{grpbg}\emph{Released RL search agents under unified exclude-seen retrieval}} \\
    \hspace{0.55em}Search-R1 (+ exclude-seen) & 40.3 & 59.6 & 64.4 & 14.0 & 7.3 & 0.3 & 37.3 & 37.3 \\
    \hspace{0.55em}Search-R1, abstention prompt (+ exclude-seen) & 42.8 & 59.8 & 66.0 & 11.8 & 6.1 & 34.7 & 42.7 & 37.8 \\
    \hspace{0.55em}ZeroSearch (+ exclude-seen) & 55.4 & 70.4 & 74.7 & 7.4 & 4.3 & 0.2 & 35.1 & 35.1 \\
    \hspace{0.55em}AutoRefine, Instruct (+ exclude-seen) & 44.4 & 63.3 & 71.8 & 13.5 & 8.3 & 0.1 & 42.9 & 42.9 \\
    \hspace{0.55em}AutoRefine, Base (+ exclude-seen) & 36.3 & 56.0 & 59.7 & 18.2 & 12.9 & 0.0 & 45.3 & \best{45.3} \\
    \hspace{0.55em}ReSearch (+ exclude-seen) & 32.0 & 56.4 & 70.6 & 21.6 & 8.9 & 0.0 & 40.4 & 40.4 \\
    \hspace{0.55em}R1-Searcher (+ exclude-seen) & 24.1 & 46.1 & 60.7 & 22.3 & 13.3 & 0.0 & 40.8 & 40.7 \\
    \hspace{0.55em}AWA-RL (+ exclude-seen) & 35.9 & 45.0 & 60.3 & 20.7 & 5.9 & 0.0 & 34.3 & 34.3 \\
    \midrule
    \rowcolor{grpbg}\multicolumn{9}{l}{\cellcolor{grpbg}\emph{Qwen2.5-7B defenses under unified exclude-seen retrieval}} \\
    \hspace{0.55em}Qwen2.5-7B, no defense (+ exclude-seen) & 41.0 & 57.8 & 60.1 & 7.6 & 5.7 & 48.5 & 41.4 & 34.3 \\
    \hspace{0.55em}Defensive prompt (+ exclude-seen) & 38.9 & 54.5 & 62.7 & 8.1 & 4.4 & \runnerup{52.2} & 41.1 & 32.4 \\
    \hspace{0.55em}Near-duplicate removal (+ exclude-seen) & 41.9 & 57.3 & 61.4 & 8.0 & 5.9 & 47.3 & 41.0 & 33.9 \\
    \hspace{0.55em}Provenance gate (+ exclude-seen) & 43.3 & 54.0 & 64.1 & 7.0 & 5.2 & 47.8 & 40.8 & 33.7 \\
    \hspace{0.55em}TrustRAG (+ exclude-seen) & 40.2 & 38.9 & \best{24.6} & 10.8 & 9.5 & 49.8 & 40.8 & 33.6 \\
    \midrule
    \rowcolor{grpbg}\multicolumn{9}{l}{\cellcolor{grpbg}\emph{\method{} with and without exclude-seen retrieval}} \\
    \hspace{0.55em}Qwen2.5-7B + \textbf{\method{}} (w/o exclude-seen, 3 seeds) & 17.0 & 28.7 & 31.6 & 22.5 & 15.2 & 40.3 & 47.9 & 40.1 \\
    \hspace{0.55em}Qwen2.5-7B + \textbf{\method{}} (w/o exclude-seen train \& eval) & 15.9 & 26.1 & \runnerup{27.1} & 23.6 & 14.3 & 50.1 & \runnerup{50.2} & 40.3 \\
    \hspace{0.55em}Qwen2.5-7B + \textbf{\method{}} (+ exclude-seen, 3 seeds) & \runnerup{14.3} & \best{23.9} & 28.9 & \runnerup{25.8} & \runnerup{16.7} & 37.6 & 47.1 & 40.1 \\
    \hspace{0.55em}Llama-3.1-8B + \textbf{\method{}} (+ exclude-seen, 1 seed) & \best{11.1} & \runnerup{24.1} & 30.6 & \best{26.5} & \best{17.2} & \best{52.5} & \best{55.4} & \runnerup{44.2} \\


==> sections/table_app_horizon.tex <==
    \rowcolor{grpbg}\multicolumn{10}{l}{\cellcolor{grpbg}\emph{Search-R1}} \\
    \hspace{0.55em}$B{=}4,\ k{=}3$ (default) & 2.52 & 1.94 & 26.3 & 46.0 & 63.3 & 69.1 & 13.3 & 6.8 & 0.2 \\
    \hspace{0.55em}$B{=}6,\ k{=}3$ & 2.65 & 2.00 & 27.2 & 48.9 & 66.4 & 65.7 & 13.7 & 7.2 & 0.3 \\
    \hspace{0.55em}$B{=}8,\ k{=}3$ & 2.71 & 2.02 & 26.5 & 50.1 & 62.0 & 66.2 & 13.8 & 7.9 & 0.1 \\
    \hspace{0.55em}$B{=}8,\ k{=}3$ (+ exclude-seen) & 2.82 & 2.03 & 26.6 & 44.0 & 58.5 & 67.4 & 14.1 & 7.0 & 0.3 \\
    \hspace{0.55em}$B{=}4,\ k{=}5$ & 2.36 & 1.80 & 26.5 & 49.9 & 62.6 & 72.1 & 14.5 & 6.7 & 0.1 \\
    \midrule
    \rowcolor{grpbg}\multicolumn{10}{l}{\cellcolor{grpbg}\emph{AutoRefine (Base)}} \\
    \hspace{0.55em}$B{=}4,\ k{=}3$ (default) & 2.22 & 1.90 & 33.0 & 40.5 & 57.2 & 59.8 & 18.1 & 12.5 & 0.0 \\
    \hspace{0.55em}$B{=}6,\ k{=}3$ & 2.24 & 1.90 & 32.7 & 39.1 & 57.7 & 61.3 & 17.9 & 12.2 & 0.0 \\
    \hspace{0.55em}$B{=}8,\ k{=}3$ & 2.24 & 1.90 & \runnerup{33.3} & 39.7 & 57.1 & 61.1 & 18.0 & 12.8 & 0.0 \\
    \hspace{0.55em}$B{=}8,\ k{=}3$ (+ exclude-seen) & 2.23 & 1.91 & 33.0 & 38.0 & 56.5 & 59.8 & 18.8 & 13.1 & 0.0 \\
    \hspace{0.55em}$B{=}4,\ k{=}5$ & 2.16 & 1.86 & \best{33.9} & 33.6 & 51.1 & 63.4 & 21.2 & 11.2 & 0.0 \\
    \midrule
    \rowcolor{grpbg}\multicolumn{10}{l}{\cellcolor{grpbg}\emph{AWA-RL}} \\
    \hspace{0.55em}$B{=}4,\ k{=}3$ (default) & 3.19 & 3.01 & 24.3 & 48.4 & 55.6 & 58.6 & 19.8 & 6.0 & 0.0 \\
    \hspace{0.55em}$B{=}6,\ k{=}3$ & 3.86 & 3.38 & 28.7 & 43.9 & 57.4 & 63.0 & 19.6 & 7.5 & 0.2 \\
    \hspace{0.55em}$B{=}8,\ k{=}3$ & 4.26 & 3.55 & 30.4 & 49.5 & 60.0 & 67.2 & 21.9 & 6.4 & 0.5 \\
    \hspace{0.55em}$B{=}8,\ k{=}3$ (+ exclude-seen) & 4.38 & 3.65 & 29.2 & 38.4 & 53.3 & 61.8 & 25.6 & 8.1 & 0.6 \\
    \hspace{0.55em}$B{=}4,\ k{=}5$ & 3.13 & 2.86 & 24.8 & 42.4 & 54.7 & 63.6 & 23.1 & 5.7 & 0.0 \\
    \midrule
    \rowcolor{grpbg}\multicolumn{10}{l}{\cellcolor{grpbg}\emph{Forced multi-turn verification baselines ($B{=}4,\ k{=}3$)}} \\
    \hspace{0.55em}Qwen2.5-7B + verify prompt (+ xs) & 1.80 & 1.46 & 20.3 & 40.7 & 62.3 & 64.8 & 10.6 & 5.1 & 34.7 \\
    \hspace{0.55em}Qwen2.5-7B + verify, min 3 turns (+ xs) & 3.01 & 3.01 & 21.1 & 26.7 & 36.5 & 54.1 & 27.5 & 7.8 & 32.1 \\
    \hspace{0.55em}Search-R1, min 3 turns (+ exclude-seen) & 3.35 & 3.18 & 24.7 & 20.2 & 36.0 & 55.5 & \runnerup{29.5} & 11.0 & 0.1 \\
    \hspace{0.55em}Search-R1 + verify, min 3 turns (+ xs) & 3.30 & 3.19 & 23.4 & 18.9 & 35.7 & 58.7 & 28.1 & 9.8 & 22.4 \\
    \hspace{0.55em}AutoRefine (Base), min 3 turns (+ xs) & 2.28 & 1.95 & 33.1 & 32.1 & 49.9 & 53.8 & 19.7 & 14.3 & 0.0 \\
    \midrule
    \rowcolor{grpbg}\multicolumn{10}{l}{\cellcolor{grpbg}\emph{\method{} (Qwen2.5-7B, 3 seeds)}} \\
    \hspace{0.55em}$B{=}4,\ k{=}3$ (+ exclude-seen, default) & 2.71 & 2.81 & 27.3 & 14.3 & 23.9 & \best{28.9} & 25.8 & 16.7 & 37.6 \\
    \hspace{0.55em}$B{=}6,\ k{=}3$ (+ exclude-seen) & 2.92 & 3.02 & 28.6 & \best{12.6} & 23.1 & 31.1 & 28.0 & 17.7 & \runnerup{43.2} \\
    \hspace{0.55em}$B{=}8,\ k{=}3$ (+ exclude-seen) & 3.00 & 3.07 & 27.5 & \runnerup{13.5} & \runnerup{22.1} & 29.8 & 28.1 & \runnerup{18.3} & \best{43.6} \\
    \hspace{0.55em}$B{=}4,\ k{=}5$ (+ exclude-seen) & 2.60 & 2.65 & 28.7 & 13.9 & \best{17.1} & \runnerup{29.1} & \best{34.8} & \best{20.2} & 34.9 \\


==> sections/table_app_l4.tex <==
    \rowcolor{grpbg}\multicolumn{11}{l}{\cellcolor{grpbg}\emph{Released search agents}} \\
    \hspace{0.55em}Search-R1 & 39.9 & 60.7 & 40.0 & 38.8 & 33.1 & 17.2 & 39.2 & 38.4 & 38.4 & 38.4 \\
    \hspace{0.55em}ZeroSearch & 38.8 & 61.7 & 37.9 & 33.3 & 32.0 & 11.2 & 31.2 & 35.1 & 35.2 & 35.2 \\
    \hspace{0.55em}AutoRefine (Instruct) & 43.5 & 62.8 & 42.2 & 42.5 & 40.2 & 21.6 & 44.0 & \runnerup{42.4} & 42.4 & 42.4 \\
    \hspace{0.55em}AutoRefine (Base) & \runnerup{47.7} & 64.8 & 45.6 & 46.5 & 38.9 & 22.5 & 47.2 & \best{44.7} & 44.7 & \best{44.7} \\
    \hspace{0.55em}ReSearch & 38.7 & 61.9 & 42.7 & 42.6 & 36.1 & 22.7 & 39.2 & 40.6 & 40.6 & 40.6 \\
    \hspace{0.55em}R1-Searcher & 38.4 & 59.2 & 35.6 & 45.5 & \runnerup{45.8} & 22.2 & 45.6 & 41.7 & 41.8 & 41.7 \\
    \hspace{0.55em}AWA-RL & 31.3 & 55.2 & 40.2 & 37.8 & 27.7 & 15.9 & 43.2 & 35.8 & 35.9 & 35.9 \\
    \midrule
    \rowcolor{grpbg}\multicolumn{11}{l}{\cellcolor{grpbg}\emph{Qwen2.5-7B with inference-time defenses}} \\
    \hspace{0.55em}No defense & 39.0 & 65.1 & 44.7 & 40.3 & 33.2 & 18.8 & 36.4 & 28.8 & 41.1 & 33.8 \\
    \hspace{0.55em}TrustRAG & 37.7 & 63.4 & 43.7 & 39.8 & 32.9 & 18.9 & 35.5 & 28.0 & 40.3 & 33.0 \\
    \hspace{0.55em}MADAM-RAG$^\dagger$ & 46.3 & 74.5 & 58.9 & 51.4 & 32.3 & 28.9 & 47.6 & 18.9 & 55.7 & 28.3 \\
    \midrule
    \rowcolor{grpbg}\multicolumn{11}{l}{\cellcolor{grpbg}\emph{Qwen2.5-7B trained on the same questions}} \\
    \hspace{0.55em}Exact-match RL & 37.2 & 60.6 & 36.8 & 38.0 & 31.6 & 19.6 & 36.0 & 36.5 & 37.2 & 36.8 \\
    \hspace{0.55em}$\lambda$-reward RL & 37.8 & 63.9 & 45.1 & 41.4 & 37.0 & 20.3 & 45.6 & 33.8 & 42.4 & 37.6 \\
    \hspace{0.55em}\textbf{\method{}} (3 seeds) & 42.5 & \runnerup{66.7} & \runnerup{47.6} & \runnerup{49.0} & 42.5 & \runnerup{28.5} & \runnerup{48.0} & 34.9 & \runnerup{47.1} & 40.1 \\
    \midrule
    \rowcolor{grpbg}\multicolumn{11}{l}{\cellcolor{grpbg}\emph{Llama-3.1-8B cross-family replication (1 seed)}} \\
    \hspace{0.55em}No defense & 29.4 & 51.5 & 35.6 & 26.7 & 18.1 & 10.5 & 26.2 & 26.8 & 28.4 & 27.6 \\
    \hspace{0.55em}Exact-match RL & 41.7 & 64.5 & 40.5 & 39.9 & 41.3 & 21.6 & \runnerup{48.0} & 41.7 & 42.7 & 42.2 \\
    \hspace{0.55em}\textbf{\method{}} & \best{48.2} & \best{71.6} & \best{55.6} & \best{56.5} & \best{56.6} & \best{36.7} & \best{56.7} & 36.7 & \best{55.4} & \runnerup{44.2} \\
    \midrule
    \rowcolor{grpbg}\multicolumn{11}{l}{\cellcolor{grpbg}\emph{Qwen2.5-7B with orthogonal retrieval filters (3 seeds)}} \\
    \hspace{0.55em}\textbf{\method{}} + TrustRAG & 40.4 & 65.2 & 46.6 & 47.1 & 36.2 & 26.3 & 42.5 & 34.0 & 44.1 & 38.3 \\
    \hspace{0.55em}\textbf{\method{}} + Sem.\ dedup & 42.2 & 66.1 & 49.2 & 46.9 & 40.1 & 26.2 & 47.4 & 35.3 & 46.2 & 40.0 \\


==> sections/table_app_worlds.tex <==
    \rowcolor{grpbg}\multicolumn{11}{l}{\cellcolor{grpbg}\emph{Test Set A: Qwen3-32B generator, 507 questions $\times$ 10 worlds}} \\
    \hspace{0.55em}Search-R1 & 24.1 & 28.2 & 62.5 & 15.0 & 47.5 & 63.1 & 70.5 & 11.1 & 5.5 & 0.0 \\
    \hspace{0.55em}AutoRefine (Base) & \best{32.1} & \best{35.9} & \best{68.6} & \best{20.1} & 41.1 & 56.4 & 62.6 & 16.6 & 10.7 & 0.0 \\
    \hspace{0.55em}R1-Searcher & \runnerup{31.4} & \runnerup{34.9} & \runnerup{66.7} & \runnerup{19.5} & 35.2 & 55.4 & 64.8 & 20.7 & 11.1 & 0.0 \\
    \hspace{0.55em}AWA-RL & 23.5 & 24.5 & 47.1 & 12.2 & 52.9 & 52.9 & 57.1 & 19.7 & 4.1 & 0.0 \\
    \hspace{0.55em}Qwen2.5-7B (no defense) & 16.6 & 16.8 & 51.7 & 7.9 & 38.1 & 58.3 & 57.1 & 6.5 & 4.3 & \runnerup{50.7} \\
    \hspace{0.55em}Qwen2.5-7B + TrustRAG & 15.4 & 15.0 & 25.1 & 7.3 & 37.2 & 41.0 & \runnerup{20.5} & 12.0 & 9.1 & 48.1 \\
    \hspace{0.55em}$\lambda$-reward RL & 19.7 & 22.9 & 61.1 & 12.2 & 50.0 & 69.0 & 71.0 & 8.7 & 4.9 & 33.1 \\
    \hspace{0.55em}Qwen2.5-7B + \textbf{\method{}} & 25.9 & 29.1 & 44.2 & 13.5 & \runnerup{9.1} & \best{14.0} & \best{19.0} & \runnerup{27.7} & \runnerup{17.9} & 37.5 \\
    \hspace{0.55em}Llama-3.1-8B + \textbf{\method{}} & 27.6 & 32.4 & 44.6 & 13.6 & \best{5.7} & \runnerup{14.3} & 23.6 & \best{28.4} & \best{18.3} & \best{52.3} \\
    \arrayrulecolor[HTML]{CBD2D9}\midrule\arrayrulecolor{black}
    \hspace{0.55em}Qwen2.5-7B + \textbf{\method{}} + TrustRAG & 25.4 & 23.4 & 28.3 & 13.7 & 10.3 & \best{12.4} & \best{10.1} & \runnerup{31.8} & \runnerup{19.9} & 37.2 \\
    \hspace{0.55em}Qwen2.5-7B + \textbf{\method{}} + Sem.\ dedup & 25.3 & 28.8 & 47.3 & 13.1 & 9.5 & 19.0 & 22.1 & \best{39.1} & \best{22.0} & 33.7 \\
    \midrule
    \rowcolor{grpbg}\multicolumn{11}{l}{\cellcolor{grpbg}\emph{Test Set B: Phi-4 generator, unseen family, 607 questions $\times$ 10 worlds}} \\
    \hspace{0.55em}Search-R1 & 28.5 & 32.6 & 50.7 & 19.3 & 44.5 & 63.6 & 67.6 & 15.5 & 8.1 & 0.3 \\
    \hspace{0.55em}AutoRefine (Base) & \best{33.8} & \best{37.7} & \runnerup{57.2} & \best{23.1} & 40.0 & 58.0 & 57.1 & 19.6 & 14.3 & 0.0 \\
    \hspace{0.55em}R1-Searcher & \runnerup{32.6} & \best{37.7} & \best{57.5} & \runnerup{21.6} & 31.3 & 53.0 & 59.1 & 21.2 & 14.0 & 0.0 \\
    \hspace{0.55em}AWA-RL & 25.2 & 30.3 & 47.5 & 16.0 & 43.8 & 58.2 & 60.1 & 19.9 & 7.9 & 0.0 \\
    \hspace{0.55em}Qwen2.5-7B (no defense) & 18.8 & 21.1 & 42.5 & 10.2 & 45.6 & 56.1 & 60.5 & 7.7 & 6.8 & \runnerup{47.8} \\
    \hspace{0.55em}Qwen2.5-7B + TrustRAG & 17.1 & 16.0 & 20.8 & 9.6 & 33.6 & 42.3 & \best{25.0} & 10.7 & 9.7 & \runnerup{47.8} \\
    \hspace{0.55em}$\lambda$-reward RL & 22.6 & 27.4 & 50.1 & 15.0 & 40.9 & 67.9 & 67.9 & 10.2 & 5.4 & 32.0 \\
    \hspace{0.55em}Qwen2.5-7B + \textbf{\method{}} & 28.6 & 31.9 & 43.3 & 16.9 & \runnerup{19.4} & \best{33.8} & 38.8 & \runnerup{24.0} & \runnerup{15.4} & 37.6 \\
    \hspace{0.55em}Llama-3.1-8B + \textbf{\method{}} & 30.1 & \runnerup{34.9} & 45.1 & 18.1 & \best{16.4} & \runnerup{33.9} & \runnerup{37.7} & \best{24.6} & \best{16.0} & \best{52.7} \\
    \arrayrulecolor[HTML]{CBD2D9}\midrule\arrayrulecolor{black}
    \hspace{0.55em}Qwen2.5-7B + \textbf{\method{}} + TrustRAG & 27.3 & 27.0 & 27.6 & 16.9 & 17.4 & \best{26.5} & \best{15.5} & \runnerup{27.1} & \runnerup{18.2} & 35.7 \\
    \hspace{0.55em}Qwen2.5-7B + \textbf{\method{}} + Sem.\ dedup & 28.2 & 30.8 & 42.4 & 17.3 & 23.8 & \runnerup{32.8} & 35.2 & \best{33.3} & \best{18.3} & 34.1 \\


==> sections/table_app_xret.tex <==
    \rowcolor{grpbg}\multicolumn{10}{l}{\cellcolor{grpbg}\emph{Zero-shot transfer to unseen dense retriever: BAAI/bge-base-en-v1.5}} \\
    \hspace{0.55em}Search-R1 & 2.56 & 1.97 & 26.7 & 53.3 & 65.3 & 72.2 & 11.6 & 6.1 & 0.3 \\
    \hspace{0.55em}Search-R1 (+ exclude-seen) & 2.60 & 1.97 & 27.0 & 45.9 & 62.6 & 71.0 & 12.3 & 6.3 & 0.3 \\
    \hspace{0.55em}AutoRefine (Base) & 2.20 & 1.87 & \runnerup{31.7} & 41.3 & 62.4 & 65.3 & 13.2 & 10.3 & 0.0 \\
    \hspace{0.55em}AutoRefine, Base (+ exclude-seen) & 2.19 & 1.88 & \best{32.1} & 37.3 & 59.8 & 66.1 & 13.4 & 10.2 & 0.0 \\
    \hspace{0.55em}R1-Searcher & 2.51 & 2.27 & 31.5 & 34.5 & 57.0 & 61.3 & 20.9 & 11.6 & 0.1 \\
    \hspace{0.55em}R1-Searcher (+ exclude-seen) & 2.52 & 2.29 & 30.8 & 22.7 & 50.5 & 62.2 & 20.8 & 11.5 & 0.0 \\
    \hspace{0.55em}AWA-RL (+ exclude-seen) & 3.19 & 3.02 & 23.9 & 27.8 & 43.5 & 58.1 & 21.2 & 5.6 & 0.2 \\
    \hspace{0.55em}Qwen2.5-7B (no defense) & 1.22 & 1.10 & 14.8 & 40.8 & 58.9 & 61.7 & 6.1 & 4.7 & 48.5 \\
    \hspace{0.55em}Qwen2.5-7B + TrustRAG & 1.23 & 1.21 & 13.5 & 39.3 & 49.8 & \best{20.7} & 9.8 & 8.2 & \runnerup{49.0} \\
    \hspace{0.55em}Qwen2.5-7B + Exact-match RL (1 seed) & 2.51 & 2.01 & 25.8 & 37.6 & 58.4 & 67.7 & 14.3 & 7.6 & 1.3 \\
    \hspace{0.55em}Qwen2.5-7B + \textbf{\method{}} (+ xs, 3 seeds) & 2.80 & 2.92 & 26.9 & \runnerup{13.4} & \runnerup{21.2} & \runnerup{29.4} & \best{26.0} & \runnerup{15.2} & 36.3 \\
    \hspace{0.55em}Qwen2.5-7B + \textbf{\method{}} (w/o xs, 1 seed) & 2.71 & 2.84 & 27.6 & 19.6 & 31.8 & 34.3 & 21.5 & 14.2 & 33.7 \\
    \hspace{0.55em}Llama-3.1-8B (no defense) & 3.04 & 2.16 & 17.2 & 31.1 & 67.4 & 67.2 & 11.2 & 4.1 & 6.0 \\
    \hspace{0.55em}Llama-3.1-8B + \textbf{\method{}} (+ xs, 1 seed) & 2.60 & 2.81 & 29.3 & \best{11.3} & \best{20.8} & 30.5 & \runnerup{25.2} & \best{15.4} & \best{51.8} \\
    \midrule
    \rowcolor{grpbg}\multicolumn{10}{l}{\cellcolor{grpbg}\emph{Zero-shot transfer to lexical sparse retriever: Okapi BM25}} \\
    \hspace{0.55em}Search-R1 & 2.75 & 1.94 & 22.8 & 49.2 & 63.1 & 64.1 & 9.9 & 6.1 & 0.3 \\
    \hspace{0.55em}Search-R1 (+ exclude-seen) & 2.81 & 1.94 & 22.4 & 38.2 & 58.6 & 64.8 & 11.9 & 6.3 & 0.0 \\
    \hspace{0.55em}AutoRefine (Base) & 2.29 & 1.81 & 28.9 & 44.8 & 60.4 & 67.8 & 13.3 & 9.3 & 0.0 \\
    \hspace{0.55em}AutoRefine, Base (+ exclude-seen) & 2.30 & 1.80 & \best{29.4} & 37.0 & 58.5 & 66.8 & 14.0 & 10.0 & 0.0 \\
    \hspace{0.55em}R1-Searcher & 2.62 & 2.30 & 27.0 & 41.7 & 53.5 & 59.8 & 17.5 & 10.8 & 0.3 \\
    \hspace{0.55em}R1-Searcher (+ exclude-seen) & 2.66 & 2.31 & \runnerup{29.0} & 26.7 & 47.7 & 60.5 & 19.8 & 11.5 & 0.2 \\
    \hspace{0.55em}AWA-RL (+ exclude-seen) & 3.33 & 3.04 & 20.2 & 34.7 & 46.6 & 53.6 & 20.9 & 5.8 & 0.0 \\
    \hspace{0.55em}Qwen2.5-7B (no defense) & 1.28 & 1.10 & 15.1 & 46.4 & 56.6 & 60.6 & 5.6 & 4.7 & 50.5 \\
    \hspace{0.55em}Qwen2.5-7B + TrustRAG & 1.29 & 1.28 & 15.0 & 42.3 & 47.7 & 33.4 & 7.5 & 7.3 & \runnerup{53.0} \\
    \hspace{0.55em}Qwen2.5-7B + Exact-match RL (1 seed) & 2.70 & 2.05 & 24.3 & 40.7 & 58.2 & 68.0 & 12.6 & 7.1 & 1.7 \\
    \hspace{0.55em}Qwen2.5-7B + \textbf{\method{}} (+ xs, 3 seeds) & 3.07 & 3.05 & 23.5 & \runnerup{12.2} & \runnerup{20.4} & \runnerup{25.1} & \runnerup{22.5} & \runnerup{14.4} & 34.3 \\
    \hspace{0.55em}Qwen2.5-7B + \textbf{\method{}} (w/o xs, 1 seed) & 2.94 & 2.99 & 22.9 & 20.3 & 26.7 & 29.9 & 16.4 & 12.1 & 35.6 \\
    \hspace{0.55em}Llama-3.1-8B (no defense) & 3.12 & 2.17 & 14.3 & 37.1 & 56.2 & 63.4 & 9.8 & 4.9 & 6.3 \\
    \hspace{0.55em}Llama-3.1-8B + \textbf{\method{}} (+ xs, 1 seed) & 2.88 & 2.97 & 25.2 & \best{7.9} & \best{17.1} & \best{24.0} & \best{24.4} & \best{15.5} & \best{60.1} \\


==> sections/table_main.tex <==
    \rowcolor{grpbg}\multicolumn{9}{l}{\cellcolor{grpbg}\emph{Released search agents}} \\
    \hspace{0.55em}Search-R1 & 46.0 & 63.3 & 69.1 & 13.3 & 6.8 & 0.2 & 38.4 & 38.4 \\
    \hspace{0.55em}ZeroSearch & 53.0 & 69.6 & 72.9 & 7.3 & 3.8 & 0.1 & 35.2 & 35.2 \\
    \hspace{0.55em}AutoRefine (Instruct) & 47.8 & 63.0 & 72.2 & 13.0 & 8.8 & 0.0 & 42.4 & 42.4 \\
    \hspace{0.55em}AutoRefine (Base) & 40.5 & 57.2 & 59.8 & 18.1 & 12.5 & 0.0 & 44.7 & \best{44.7} \\
    \hspace{0.55em}ReSearch & 43.5 & 64.5 & 68.9 & 20.9 & 9.4 & 0.0 & 40.6 & 40.6 \\
    \hspace{0.55em}R1-Searcher & 33.3 & 54.2 & 61.9 & 21.0 & 12.5 & 0.0 & 41.8 & 41.7 \\
    \hspace{0.55em}AWA-RL & 48.4 & 55.6 & 58.6 & 19.8 & 6.0 & 0.0 & 35.9 & 35.9 \\
    \midrule
    \rowcolor{grpbg}\multicolumn{9}{l}{\cellcolor{grpbg}\emph{Qwen2.5-7B with inference-time defenses}} \\
    \hspace{0.55em}No defense & 41.9 & 57.2 & 58.8 & 7.1 & 5.5 & 49.2 & 41.1 & 33.8 \\
    \hspace{0.55em}Defensive prompt & 42.1 & 58.3 & 61.0 & 7.9 & 4.7 & \best{52.7} & 42.0 & 32.9 \\
    \hspace{0.55em}Near-duplicate removal & 41.3 & 55.9 & 63.0 & 7.1 & 4.8 & 46.7 & 40.6 & 33.6 \\
    \hspace{0.55em}Provenance gate & 44.9 & 56.1 & 59.4 & 7.6 & 5.8 & 46.8 & 41.0 & 33.9 \\
    \hspace{0.55em}TrustRAG & 35.4 & 41.7 & \best{22.8} & 11.4 & 9.4 & 48.0 & 40.3 & 33.0 \\
    \hspace{0.55em}MADAM-RAG$^\dagger$ & 7.4 & 40.6 & 48.4 & 7.0 & 2.8 & 84.4 & 55.7 & 28.3 \\
    \midrule
    \rowcolor{grpbg}\multicolumn{9}{l}{\cellcolor{grpbg}\emph{Qwen2.5-7B trained on the same questions}} \\
    \hspace{0.55em}Exact-match RL & 35.2 & 59.5 & 67.7 & 15.9 & 8.1 & 1.4 & 37.2 & 36.8 \\
    \hspace{0.55em}$\lambda$-reward RL & 45.4 & 68.4 & 69.4 & 9.4 & 5.2 & 32.5 & 42.4 & 37.6 \\
    \hspace{0.55em}\textbf{\method{}} (3 seeds) & \runnerup{14.3} & \best{23.9} & \runnerup{28.9} & \runnerup{25.8} & \runnerup{16.7} & 37.6 & \runnerup{47.1} & 40.1 \\
    \midrule
    \rowcolor{grpbg}\multicolumn{9}{l}{\cellcolor{grpbg}\emph{Llama-3.1-8B cross-family replication (1 seed)}} \\
    \hspace{0.55em}No defense & 37.3 & 67.5 & 70.0 & 10.8 & 3.8 & 5.0 & 28.4 & 27.6 \\
    \hspace{0.55em}Exact-match RL & 33.8 & 61.3 & 66.7 & 17.6 & 9.8 & 2.8 & 42.7 & 42.2 \\
    \hspace{0.55em}\textbf{\method{}} & \best{11.1} & \runnerup{24.1} & 30.6 & \best{26.5} & \best{17.2} & \runnerup{52.5} & \best{55.4} & \runnerup{44.2} \\
    \midrule
    \rowcolor{grpbg}\multicolumn{9}{l}{\cellcolor{grpbg}\emph{Qwen2.5-7B with orthogonal retrieval filters (3 seeds)}} \\
    \hspace{0.55em}\textbf{\method{}} + TrustRAG & 13.8 & \best{19.4} & \best{12.8} & \runnerup{29.4} & \runnerup{19.0} & 36.5 & 44.1 & 38.3 \\
    \hspace{0.55em}\textbf{\method{}} + Sem.\ dedup & 16.7 & 25.9 & 28.7 & \best{36.2} & \best{20.2} & 33.9 & 46.2 & 40.0 \\

